Conic Frameworks Infinitesimal Rigidity

This paper introduces new structures called conic frameworks and their rigidity. They are composed by agents and a set of directed constraints between pairs of agents. When the structure cannot be flexed while preserving the constraints, it is said to be rigid. If only smooth deformations are considered a sufficient condition for rigidity is called infinitesimal rigidity. In conic frameworks, each agent $u$ has a spatial position $x_u$ and a clock offset represented by a bias $\beta_u$. If the constraint from Agent $u$ to Agent $w$ is in the framework, the pseudo-range from $u$ to $w$, defined as ${\left\lVert{x_u - x_w}\right\rVert} + \beta_w - \beta_u$, is set. Pseudo-ranges appear when measuring inter-agent distances using a Time-of-Arrival method. This paper completely characterizes infinitesimal rigidity of conic frameworks whose agents are in general position. Two characterizations are introduced: one for unidimensional frameworks, the other for multidimensional frameworks. They both rely on the graph of constraints and use a decoupling between space and bias variables. In multidimensional cases, this new conic paradigm sharply reduces the minimal number of constraints required to maintain a formation with respect to classical Two-Way Ranging methods.

==> old_proof_lemma_independence.tex <==
Let $\tilde \Gamma = G \cup H$ with $G$ is independent in $\R^d$ and $H$ is a spanning forest. Consider $(\Gamma,p)$ a generic conic framework whose underlying conic graph is $\tilde \Gamma$ and let us prove that the rows of the rigidity matrix $M(\Gamma, p)$ are independent. We choose the directions of the arcs in $\Gamma$ to have the arcs stemmed from $H$ satisfy $uv \in E_H \implies u > v$. Order the rows of $M(\Gamma,p)$ starting by those of $G$ then those of $H$. Consider a vector $\omega = \begin{pmatrix}-\omega_G^\intercal & \omega_H^\intercal\end{pmatrix}^\intercal$, with $\omega_G \in \R^{\card{E_G}}$ and $\omega_H\in \R^{\card{E_H}}$ inducing a null combination of the rows, \ie{} $M(\Gamma,p)^\intercal \omega = 0$. Let us prove that $\omega = 0$. As $G$ is independent the rows of the Euclidean rigidity matrix $M_e(G, p)$ are independent. Therefore, the rows of the conic rigidity matrix $M(G, p)$ are also independent. Consequently proving that $\omega_H = 0$ is sufficient. Let us prove that $\omega_H = 0$.
	
	To prove that $\omega_H = 0$, we will introduce a special ordering of the vertices and of the edges of $H$. Then, we will prove by induction that: $\forall u \in \set{1, \dots, \card{E_H}}$,
	\begin{equation}\label{eq: Induction equation lemma}
		\omega_H(u) = \sum_{j > u} b_{u, v} \omega_H(j)
	\end{equation}
	where $\omega_H(j)$ denotes the coefficient associated $j$-th edge of $H$ and the $b_{u,j}$ are scalars belonging to a field $\K_u$ to be defined. With that property proved, we will get that $\omega_H(\card{E_H}) = 0$, then by a trivial induction that $\omega_H = 0$.
	
	First, let us define the orderings on the vertices and the edges of $H$. The edges and the $\card{E_H}$ first vertices are defined by the following induction preserving the forest structure of $H$. At each step $i$, select an edge connected to a leaf in the forest, number both the edge and the leaf with index $i$ and remove them from $H$. Finally, order the remaining vertices arbitrarily. Those notations are depicted in Figure \ref{fig: Ordering spanning forest}. Note that these ordering are not unique. The interest of these two ordering is to give a triangular structure to the matrix $B(H, p)$. For example, with the forest represented in Figure \ref{fig: Ordering spanning forest}:
	\begin{equation}
		B(H, p) = \begin{bmatrix}
			d_{1,8} & 0 & 0 & 0 & 0 & 0 & 0 & -d_{1,8} \\
			0 & d_{2,6} & 0 & 0 & 0 & -d_{2,6} & 0 & 0 \\
			0 & 0 & d_{3,5} & 0 & -d_{3,5} & 0 & 0 & 0 \\
			0 & 0 & 0 & d_{4,5} & -d_{4,5} & 0 & 0 & 0 \\
			0 & 0 & 0 & 0 & d_{5,8} & 0 & 0 & -d_{5,8}
		\end{bmatrix}
	\end{equation}
	
	\begin{figure}
		\centering
		\resizebox{0.75\linewidth}{!}{\input{fig/ordering_spanning_forest.pgf}}
		\caption{Example of orderings defined in the proof of Lemma \ref{lem: Independence union minimally rigid with forest} for a spanning forest with $8$ vertices. The last three vertices are arbitrary ordered as $\card{E_H} = 5$.}
		\label{fig: Ordering spanning forest}
	\end{figure}

	Secondly, let us define the fields $\K_i$. The first field $\K_0 = \Q\left(x_{1}^{(1)}, \dots, x_{n}^{(d)}\right)$ is the field of rational in the coordinates of the points. Then by induction $\K_i$ is the extension defined as $\K_i = \K_{i-1}[d_{i, i+1}, \dots, d_{i, n}]$ where $d_{i,j}$ is the Euclidean distance between $x_{i}$ and $x_{j}$. In other words, if we denote $E_i = \set{iv \mid i < v \le n}$ then:
	\begin{equation}
		\K_i = \set{\sum_{F \in \rP(E_i)} \alpha_F \prod_{iv \in F} d_{i, v} \mid \forall F, \alpha_F \in \K_{i-1}}
	\end{equation}

	Let us now prove the induction. We only prove the inductive step as the initialization is just an special case. Let $0 \le i \le \card{E_H}$ and assume that for $u \in \set{1, \dots, i-1}$ \eqref{eq: Induction equation lemma} holds. Let us prove that \eqref{eq: Induction equation lemma} also hold for $u = i$.
	
	First, let us develop the hypothesis $M(\Gamma, p)^\intercal \omega = 0$:
	\begin{equation}
		\omega^\intercal M(\Gamma, p) =
		\begin{pmatrix}
			-\omega_G^\intercal & \omega_H^\intercal
		\end{pmatrix}
		\begin{bmatrix}
			M_e(G, p) & B(G, p) \\
			M_e(H, p) & B(H, p)
		\end{bmatrix} = 0
	\end{equation}
	This equation can be decoupled into the two following.
	\begin{align}\label{eq: the Independence equalities rigidity matrix}
		M_e(G, p)^\intercal \omega_G &= M_e(H, p)^\intercal \omega_H & 	B(G, p)^\intercal \omega_G &= B(H,p)^\intercal \omega_H
	\end{align}
	The $i$-th row of the second equation in \eqref{eq: the Independence equalities rigidity matrix} gives:
	\begin{equation}\label{eq: lem Independence 1}
		\sum_{v\in \rN_H(i)}\pm d_{i, v} \omega_H\left(l_H(i, v)\right) = \sum_{v\in \rN_{G}(i)}\pm d_{i, v} \omega_G\left(l_G(i, v)\right)
	\end{equation}
	where $\rN_H(i)$ and $\rN_{G}(i)$ denote the neighbors of $i$ in $H$ and $G$, $l_H(u,v)$ and $l_G(u,v)$ denote the index of the row corresponding to the edge between $u$ and $v$ in $H$ and $G$ and, the $\pm$ signs depend on the orientation of the arcs in $\Gamma$. It is easy to prove that $l_H(u, v) = \min(u,v)$.	The orderings also impose that the vertex $i$ is adjacent in $H$ to only one vertex of higher index, we note this index $n(i)$. For example, in the forest of Figure \ref{fig: Ordering spanning forest} $n(2) = 6$ and $n(5) = 8$. Consequently, \eqref{eq: lem Independence 1} becomes:
	\begin{equation}\label{eq: the Independence main equation}
		 d_{i, n(i)} \omega_H(i) - \sum_{\substack{v\in \rN_H(i)\\
		 		v < i}}d_{i, v} \omega_H(v) = \sum_{v\in \rN_{G}(i)}\pm d_{i, v} \omega_G\left(l_G(i, v)\right)
	\end{equation}
	
	Then by induction hypotheses, exists a family of scalars $f_{v, j} \in \K_{i-1}$ s.t. $\forall v < i$, $\omega_H(v) = \sum_{j \ge i} f_{v, j} \omega_H(j)$. We deduce that:
	\begin{equation}\label{eq: the Independence left hand side}
		\sum_{\substack{v\in \rN_H(u_i)\\
				v < i}}d_{i, v} \omega_H(v) = \sum_{j \ge i} g_{j} \omega_H(j)
	\end{equation} 
	with:
	\begin{equation*}
		g_j = \sum_{\substack{v\in \rN_H(u_i)\\
				v < i}}d_{i, v} f_{v, j} \in \K_{i-1}
	\end{equation*}

	Now let us focus on the right hand side of \eqref{eq: the Independence main equation}. Since, $G$ is independent, by definition so are the rows of $M_e(G, p)$. The first equation in \eqref{eq: the Independence equalities rigidity matrix} gives that $\omega_G = A \omega_H$ with:
	\begin{equation}\label{eq: lem Independance definition of A}
		A = \left(M_e(G, p)M_e(G, p)^\intercal\right)^{-1}M_e(G, p)M_e(H, p)^\intercal
	\end{equation}
	We note that $a_{i,j}$, the entry of $A$ at the $i$-th row and $j$-rh column, belongs to $\K_0$. The right hand side of \eqref{eq: the Independence main equation} becomes:
	\begin{equation}
		\sum_{v\in \rN_{G}(i)}\pm d_{i, v} \omega_G\left(l_G(i, v)\right) = \sum_{j=1}^{\card{E_H}}\sum_{v\in \rN_{G}(i)}\pm d_{i, v} a_{l_G(i, v), j}\omega_H(j)
	\end{equation}
	Similarly as before, we use induction hypotheses to replace the terms in $\omega_H(j)$ with $j < i$ and we get:
	\begin{equation}\label{eq: the Independence right hand side}
		\sum_{v\in \rN_{G}(i)}\pm d_{i, v} \omega_G\left(l_G(i, v)\right) = \sum_{j = i}^{\card{E_H}}h_j\omega_H(j)
	\end{equation}
	where:
	\begin{equation}
		h_j = \sum_{v\in \rN_{G}(i)}\pm d_{i, v} \left[a_{l_G(i, v), j} + \sum_{j_0 = 0}^{i - 1} a_{l_G(i, v), j_0}f_{j_0, j} \right] \in \K_i
	\end{equation}
	Substituting \eqref{eq: the Independence left hand side} and \eqref{eq: the Independence right hand side} in \eqref{eq: the Independence main equation} gives:
	\begin{equation}
		b'_{i,i} \omega_H(i) = \sum_{j > i} b'_{i,j} \omega_H(j)
	\end{equation}
	with:
	\begin{align}
		b'_{i,i} &= d_{i, n(i)} - g_i -  \sum_{v\in \rN_{G}(i)}\pm d_{i, v} \left[a_{l_G(i, v), i} + \sum_{j_0 < i} a_{l_G(i, v), j_0}f_{j_0, i} \right] \in \K_i \label{eq: lem Independence expression b'_{i,i}} \\
		b'_{i,j} &= g_j + h_j \in \K_i
	\end{align}
	If $b'_{i,i} \neq 0$, we conclude by setting $b_{i,j} = b'_{i,j}/b'_{i,i}$. Let us finally prove that $b'_{i,i} \neq 0$.
	
	The field $\K_i = \K_{i-1}[d_{i, i+1}, \dots, d_{i, n}]$ is a $\K_{i-1}$ vector space whose natural basis is $\set{\prod_{iv \in F} d_{i, v} \mid F \in \rP(E_i)}$. The scalar $b'_{i,i} \in \K_i$, we claim that the coordinates of $b'_{i,i}$ in the natural base associated to basis vector $d_{i,n(i)}$ is not null. We denote $\alpha_0$ this coordinate. In \eqref{eq: lem Independence expression b'_{i,i}}, remind that $g_i \in \K_{i-1}$, the $f_{j_0, i} \in \K_{i-1}$ and the entries of $A$ also belong to $K_0 \subset K_{i-1}$. Therefore, if $n(i) \notin \rN_G(i)$, then $\alpha_0 = 1$. On the other hand, if $n(i) \in \rN_G(i)$, then the arc associated to edge $in(i)$ from $G$ is directed from $i$ to $n(i)$ (since the arc $n(i)$ to $i$ is already stemmed by $H$). Therefore:
	\begin{equation}
		\alpha_0 = 1 + a_{l_G(i, n(i)), i} + \sum_{j_0 < i} a_{l_G(i, n(i)), j_0}f_{j_0, i}
	\end{equation}
	Note that by definition of $A$ \eqref{eq: lem Independance definition of A}, $A = M_e(G,p)^+ M_e(H,p)^\intercal$ where $M_e(G,p)^+$ is left pseudo-inverse of $M_e(G,p)^\intercal$. As an interpretation, since the rows of $M_e(G,)$ are independent, the columns of $A$ represent the coordinates of 
	As a consequence, $b'_{i,i} \neq 0$ and we can indeed set $b'_{i,j} = b'_{i,j}/b'_{i,i}$.
